A Suite of Reduced-Order Models of a Single-Layer Lithium-ion Pouch Cell

For many practical applications, fully coupled three-dimensional models describing the behaviour of lithium-ion pouch cells are too computationally expensive. However, owing to the small aspect ratio of typical pouch cell designs, such models are well approximated by splitting the problem into a model for through-cell behaviour and a model for the transverse behaviour. In this paper, we combine different simplifications to through-cell and transverse models to develop a hierarchy of reduced-order pouch cell models. We give a critical numerical comparison of each of these models in both isothermal and thermal settings, and also study their performance on realistic drive cycle data. Finally, we make recommendations regarding model selection, taking into account the available computational resource and the quantities of interest in a particular study.

==> old_model_text.tex <==


\begin{comment}
\section{Asymptotic reduction of the 2+1D DFN model}\label{sec:asymptotic-reduction}
\rob{I've updated the equations above, but still need to go through the below and make changes/update broken references.}
In \cite{sulzer_part_I}, the variables were expanded in powers of $\delta^2$, where $\delta$ is the geometric aspect ratio of the cell. In the following, we consider three limiting cases. The first is the case of a small diffusion timescale in the electrolyte relative to the typical discharge timescale as well as a large ratio of the thermal voltage to the typical potential drop in the electrode and electrolyte. We refer to this as the `fast electrolyte diffusion and high electrode and electrolyte conductivity' case. In the second case, we consider the limit of a large ratio of the thermal voltage to the typical potential drop in the current collectors, which we refer to as the `high current collector conductance' case. Finally, we consider the combination of both `fast electrolyte diffusion and high electrode and electrolyte conductivity' and `high current collector conductance'. In total, we develop six reduced-order models, with a leading order model and a first order corrected model for each limit

It is worth commenting on the coupling between the electrochemcial behaviour and the heat transport. We note that the temperature rise $\Delta T^*$ is typically in the range of $1 - \SI{10}{K}$, making the ratio of the temperature changes to the ambient temperature, $\Theta\approx 0.01$-$0.1$. If we consider $\Theta\sim \mathcal{O}(1)$ then the temperature will appear in the Butler-Volmer equation, the temperature dependent coefficients, and the open circuit potentials at leading-order. This gives rise to a coupled electrochemical--thermal problem. For small temperature increases we may wish to consider $\Theta\sim \mathcal{O}(\delta)$, in which case we find that the leading-order electrochemical problem will depend only on the ambient temperature $T^* = T^*_{\infty}$ (i.e. $T = 0$). We might then extend our analysis to first-order to include the effect the temperature has on the surface reactions. Instead in each of our limiting models, we consider $\Theta\sim \mathcal{O}(1)$ so that our reduced models describe the cell behaviour over a greater range of temperatures.

\subsection{Fast electrolyte diffusion and high electrode and electrolyte conductivity}
We first consider the case of `fast electrolyte diffusion and high electrode and electrolyte conductivity', that is, the case where the timescale for migration of lithium ions in the electrolyte is small relative to the typical timescale of a discharge and the typical potential drop in the electrode and electrolyte is small relative to the thermal voltage. This limit was also explored in \cite{Marquis2019} for the case of a 1D electrochemical model. Mathematically, this corresponds to taking the limit $\delta\rightarrow 0$, with
% In the following, we reduce the model further by exploiting the small ratio of the diffusion time through the electrolyte to the typical discharge timescale, as in \cite{Marquis2019}. In particular, we consider the case $\mathcal{C}\ts{e} \sim \mathcal{O}(\delta)$. This is achieved by expanding the leading-order variables in \eqref{DFNCC}--\eqref{DFNCC:IC} in powers of $\delta$. Note that terms $\mathcal{O}(\delta^2)$ must be neglected in order to be consistent with the analysis used to derive the system \eqref{DFNCC}--\eqref{DFNCC:IC}. \\
%\begin{equation}\label{eqn:thin-or-poorly-conducting-current-collectors}
%    \mathcal{C}\ts{e}'=\frac{\mathcal{C}\ts{e}}{\delta}\sim 1, \quad
%    L\ts{cn}\sigma\ts{cn}'\sim1, \quad
%    L\ts{cp}\sigma\ts{cp}'\sim1, \quad
%    \sigma\ts{n}'=\sigma\ts{n}\delta \sim 1, \quad
%    \sigma\ts{p}'=\sigma\ts{p}\delta \sim 1, \quad
%    \hat{\kappa}\ts{e}'=\hat{\kappa}\ts{e}\delta \sim 1.
%\end{equation}
\begin{equation}\label{eqn:thin-or-poorly-conducting-current-collectors}
    \mathcal{C}\ts{e}=\delta \mathcal{C}\ts{e}' =\mathcal{O}(\delta), \quad
 %   L\ts{cn}\sigma\ts{cn}'=\mathcal{O}(1), \quad
 %   L\ts{cp}\sigma\ts{cp}'=\mathcal{O}(1), \quad
    \sigma\ts{n}=\frac{\sigma\ts{n}'}{\delta} =\mathcal{O}\left(\frac{1}{\delta}\right), \quad
        \sigma\ts{p}=\frac{\sigma\ts{p}'}{\delta} =\mathcal{O}\left(\frac{1}{\delta}\right), \quad
        \hat{\kappa}\ts{e}=\frac{\hat{\kappa}\ts{e}'}{\delta} =\mathcal{O}\left(\frac{1}{\delta}\right), 
\end{equation}
and all other parameters are $\mathcal{O}(1)$.
We then expand all variables in powers of $\delta$ in the form
\begin{equation}\label{eqn:expand}
c\ts{s,k} = c\ts{s,k}^0 + \delta c\ts{s,k}^1 + \delta^2 c\ts{s,k}^2 + \dots.
\end{equation}


\subsubsection{Leading order: 2+1D SPM} \label{sec:2p1-SPM}
%In this section, we consider the limit of fast diffusion in the electrolyte and large conductivity in the electrodes. This is the same limit  by writing $\mathcal{C}\ts{e} = \delta \mathcal{C}\ts{e}' $, $\sigma\ts{k} = \sigma\ts{k}'/\delta$ for $\kin{n, p}$, $\hat{\kappa}\ts{e} = \hat{\kappa}\ts{e}'/\delta$, where $\mathcal{C}\ts{e}$, $\sigma\ts{k}'$ and $\hat{\kappa}\ts{e}'$ are all $\mathcal{O}(1)$ quantities, but treat $\alpha \sim \mathcal{O}(1)$. This is realised in practice by having current collectors that are poorer conductors or are much thinner. Note that in this case we also have $1/(\sigma\ts{ck}A\ts{tab,k}) \sim \mathcal{O}(1)$, since $A\ts{tab,k}$ scales with $L\ts{ck}$. After rescaling $\sigma\ts{k}$, we look for a solution in terms of an asymptotic series in $\delta$, writing
%\begin{equation}
%\phi\ts{s,k} = \phi\ts{s,k}^0 + \delta \phi\ts{s,k}^1 + \cdots,
%\end{equation}
%etc.
At leading order in $\delta$, the current collector equations: (\ref{DFNCC:eqn:phi_s_cn}), (\ref{DFNCC:eqn:phi_s_cp}), (\ref{bc:nDim:reference_potential}), (\ref{bc:nDim:applied current}), and (\ref{bc:nDim:external_cc}) become
\begin{subequations}\label{eqn:leading-order-current-collector}
\begin{align}
    L\ts{cn}\sigma\ts{cn}'\nabla_\perp^2 \phi\ts{s,cn}^0 = \mathcal{I}^0 \\
    L\ts{cp}\sigma\ts{cp}'\nabla_\perp^2 \phi\ts{s,cp}^0 = -\mathcal{I}^0
\end{align}
\begin{gather}
    \phi\ts{s,cn}^0 = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{tab,n}, \\
\frac{1}{L_yL_z}\int_{\partial\Omega\ts{tab,p}}\nabla_\perp\phi\ts{s,cp}^0\cdot\boldsymbol{n} = - \frac{I_{\text{app}}}{\sigma\ts{cp}'}\\
\nabla_\perp\phi\ts{s,k}^0\cdot\boldsymbol{n} = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{ext,k} \quad \kin{cn, cp}.
\end{gather}
\end{subequations}
This problem remains coupled to the electrochemical problem with the term $\mathcal{I}^0$ to be determined as part of the solution.

Within the electrolyte, electrodes, and particles, the leading-order problem is the same as that for the 1D case studied in \cite{Marquis2019}, except for the trivial extension for thermal coupling. Therefore, we simply provide the algebraic expressions for leading-order terms in Appendix \ref{app:algebraic-expressions}. In addition to these algebraic expressions, we must also solve, in a single representative particle at each $(y,z)$ point in each electrode, the problem
\begin{subequations}\label{eqn:leading-order-particles}
\begin{gather} \label{eqn:lo:solidConcentration}
     \mathcal{C}\ts{k}\pdv{c\ts{s,k}^0}{t} = -\frac{1}{r\ts{k}^2}\pdv{r\ts{k}}
        \left(
            r\ts{k}^2 D\ts{k}(c\ts{s,k}^0, T^0)
            \pdv{c\ts{s,k}^0}{r\ts{k}}
        \right), \quad \kin{n, p} \\
    \pdv{c\ts{s,k}^0}{r\ts{k}}\bigg|_{r\ts{k}=0}=0, \quad
    -\frac{a\ts{k}\gamma\ts{k}}{\mathcal{C}\ts{k}}
        D\ts{k}(c\ts{s,k}^0, T^0)
        \pdv{c\ts{s,k}^0}{r\ts{k}}\bigg|_{r\ts{k}=0}=,
     \begin{cases}
     \frac{\mathcal{I}^0}{L\ts{n}}, \quad & \text{k}=\text{n}, \\
     -\frac{\mathcal{I}^0}{L\ts{p}}, \quad &\text{k}=\text{p},
     \end{cases} \label{eqn:lo:solidConcentration:BC} \\
     c\ts{s,k}^0(r\ts{k},0) = c\ts{s,k,0}, \quad \kin{n, p}.
     %N\ts{s,k}^0\bigg|_{r\ts{k}=0} &= 0, \quad  \kin{n p}, \ \ \frac{a\ts{k}\gamma\ts{k}}{\mathcal{C}\ts{k}}N\ts{s,k}^0\bigg|_{r\ts{k}=1} =
     %\begin{cases}
     %\frac{\mathcal{I}^0}{L\ts{n}}, \quad & \text{k}=\text{n}, \\
     %-\frac{\mathcal{I}^0}{L\ts{p}}, \quad &\text{k}=\text{p},
     %\end{cases} \label{eqn:lo:solidConcentration:BC}
     %&&\\
\end{gather}
\end{subequations}
At this order, all the particles at a particular $(y,z)$ location in an electrode behave in the same way. Therefore, we can solve \eqref{eqn:leading-order-particles} in just a single representative particle instead of in every particle in the $x$-direction.

%\begin{comment}
%In the electrolyte \eqref{eqn:nDim:electrolyte:concentration} and \eqref{eqn:nDim:electrolyte:flux} give, to leading-order,
%\begin{equation}
    %\pdv{N\ts{e,k}^0}{x} = 0, \quad N\ts{e,k}^0 = - \epsilon\ts{k}^{\text{b}} D\ts{e}(c\ts{e,k}^0,T^0) \pdv{c\ts{e,k}^0}{x}, \quad \kin{n, s, p},
%\end{equation}
%which upon application of the boundary conditions \eqref{bc:nDim:no_electrolyte_cc_flux}--\eqref{bc:nDim:concentration_continuity_Lp}, the initial condition \eqref{ic:nDim:electrolyte}, and through consideration of conservation of lithium, yields
%\begin{equation}
    %N\ts{e,k}^0 = 0, \quad c\ts{e,k}^0 = 1, \quad \kin{n, s, p}.
%\end{equation}
%The leading-order components of \eqref{eqn:nDim:McIn} and \eqref{eqn:nDim:solid:ohms} are then
%\begin{equation}\label{eqn:lo:phi_const}
	%\pdv{\phi\ts{e,k}^0}{x} = 0, \quad \pdv{\phi\ts{k}^0}{x} = 0.
%\end{equation}
%Since $c\ts{e,k}^0$, $\phi\ts{e,k}^0$, and $\phi\ts{k}^0$ are all independent of $x$, and $c\ts{k}^0$ is initially independent of $x$, it follows from the leading-order components of \eqref{eqn:nDim:BV}, \eqref{eqn:nDim:exchange_current}, and \eqref{eqn:nDim:overpotential} that $j\ts{k}^0$, $j\ts{0,k}^0$ and $\eta\ts{k}^0$ are also independent of $x$. Therefore, we may integrate \eqref{eqn:nDim:electrolyte:current} with respect to $x$ over region $\Omega\ts{k}$ for $\kin{n, p}$ and apply \eqref{bc:nDim:no_electrolyte_cc_current}--\eqref{bc:nDim:charge_continuity_Lp}, to obtain
%\begin{align}
    %\label{eqn:lo:current}
    %i\ts{e,n}^0 &= x\frac{\mathcal{I}^0}{L\ts{n}}, \quad i\ts{e,s}^0=\mathcal{I}^0, \quad i\ts{e,p}^0 = (1-x)\frac{\mathcal{I}^0}{L\ts{p}}, \\
    %\label{eqn:lo:G0}
    %&\qquad j\ts{n}^0 = \frac{\mathcal{I}^0}{L\ts{n}}, \quad j\ts{p}^0 = -\frac{\mathcal{I}^0}{L\ts{p}}.
%\end{align}
%From the \eqref{eqn:nDim:BV}, we obtain the leading-order overpotentials
%\begin{align}\label{eqn:lo:eta}
    %\eta\ts{n}^0 = 2(1 + \Theta T^0)\sinh^{-1}\left(\frac{\mathcal{I}^0}{j\ts{0,n}^0L\ts{n}} \right), \quad \eta\ts{p}^0 =-2 (1 + \Theta T^0)\sinh^{-1}\left(\frac{\mathcal{I}^0}{j\ts{0,p}^0L\ts{p}} \right).
%\end{align}
%From \eqref{eqn:lo:phi_const} and continuity of the electrical potential \eqref{bc:nDim:charge_continuity_Ln} and \eqref{bc:nDim:charge_continuity_Lp}, we find that the concentration overpotential is zero
%\begin{equation}\label{eqn:lo:concentration:overportential}
    %\phi\ts{e,p}^0 - \phi\ts{e,n}^0 = 0.
%\end{equation}
%
%The leading-order potential difference $\mathcal{V} = \phi\ts{s,cp} - \phi\ts{s,cn}$ is then
%\begin{equation}\label{eqn:asim1:VLO}
    %\mathcal{V}^0 =
    %\left.U\ts{p}(c\ts{s,p}^0, T^0)\right|_{r\ts{p}=1} - \left.U\ts{n}(c\ts{s,n}^0, T^0)\right|_{r\ts{n}=1}
    %-2(1 +\Theta T^0)\sinh^{-1}\left(\frac{\mathcal{I}^0}{j\ts{0,p}^0L\ts{p}} \right)  -2(1 +\Theta T^0)\sinh^{-1}\left(\frac{\mathcal{I}^0}{j\ts{0,n}^0L\ts{n}} \right),
%\end{equation}
%where the leading-order component of the exchange current density, as given by \eqref{eqn:nDim:exchange_current}, is
%\begin{equation}\label{eqn:lo:exchange_current}
    %j\ts{0,k}^0= \frac{\gamma\ts{k}}{\mathcal{C}\ts{r,k}} m\ts{k}(T^0) (c^0\ts{s,k})^{1/2} (1-c\ts{s,k}^0)^{1/2}.
%\end{equation}
%It then remains to find the leading-order lithium concentration in the active phase, and the temperature.
%
%Equations \eqref{eqn:nDim:solid:concentration} and \eqref{bc:nDim:particle} give the following problem describing transport of lithium in the electrode particles to leading-order
%\begin{subequations}\label{eqn:leading-order-particles}
	%\begin{align} \label{eqn:lo:solidConcentration}
     %\mathcal{C}\ts{k}\pdv{c\ts{s,k}^0}{t} &= -\frac{1}{r\ts{k}^2}\pdv{r\ts{k}}\left(r\ts{k}^2 N\ts{s,k}^0\right), \quad N\ts{s,k}^0 = D\ts{k}(c\ts{s,k}^0, T^0) \pdv{c\ts{s,k}^0}{r\ts{k}}, && \kin{n, p} \\
     %N\ts{s,k}^0\bigg|_{r\ts{k}=0} &= 0, \quad  \kin{n p}, \ \ \frac{a\ts{k}\gamma\ts{k}}{\mathcal{C}\ts{k}}N\ts{s,k}^0\bigg|_{r\ts{k}=1} =
     %\begin{cases}
     %\frac{\mathcal{I}^0}{L\ts{n}}, \quad & \text{k}=\text{n}, \\
     %-\frac{\mathcal{I}^0}{L\ts{p}}, \quad &\text{k}=\text{p},
     %\end{cases} \label{eqn:lo:solidConcentration:BC}
     %&&\\
     %c\ts{s,k}^0(r\ts{k},0) &= c\ts{s,k,0}, && \kin{n, p},
    %\end{align}
%\end{subequations}
%which must be solved for a particle at each $(y,z)$ location in both the positive and negative electrode.

At leading order, the thermal problem (\ref{DFNCC:eqn:thermal}), (\ref{DFNCC:BC:tempext}), and (\ref{ic:nDim:temp}) becomes
\begin{subequations}\label{eqn:leading-order-temperature}
\begin{gather}\label{eqn:asim1:LOtemp}
    \mathcal{C}\ts{th} \rho \pdv{T^0}{t} = \lambda \nabla_\perp^2T^0 + \mathcal{B}\bar{Q}^0 - \frac{2 h'}{L} T^0    \\
    \nabla_\perp T^0 \cdot \boldsymbol{n} = 0, \quad T^0(y,z,0) =T_0
\end{gather}
where the $x$-averaged leading-order heat generation term is computed from the expansions provided in Appendix~\ref{app:heatgen}, and reads
\begin{equation}
\begin{split}
       \bar{Q}^0 &= \frac{1}{L}\bigg[ L\ts{cn}\sigma\ts{cn}'\vert \nabla_\perp \phi\ts{cn}^0 \vert^2 + L\ts{cp}\sigma\ts{cp}'\vert \nabla_\perp \phi\ts{cp}^0 \vert^2 \\
       &\quad +  L\ts{n} j\ts{n}^0\left( \eta\ts{n}^0 + (\Theta^{-1} + T^0)\pdv{U\ts{n}}{T}\bigg\vert_{T=0} \right) + L\ts{p} j\ts{p}^0\left( \eta\ts{p}^0 + (\Theta^{-1} + T^0)\pdv{U\ts{p}}{T}\bigg\vert_{T=0} \right)\bigg].
\end{split}
\end{equation}
\end{subequations}
Equations (\ref{eqn:leading-order-current-collector}), (\ref{eqn:leading-order-particles}), (\ref{eqn:leading-order-temperature}), and (\ref{eqn:leading-order-internals}) form the complete leading-order model. The model retains the 2+1D structure of the 2+1D DFN but replaces the through-cell 1D electrochemical model by the commonly used SPM \cite{Moura2017, bizeray2018identifiability, guo2011single, dey2014combined, reniers2019review}. For this reason, we refer to this model as the 2+1D SPM.

\subsubsection{First order correction:2+1D SPM}\label{sec:poor-cc-first-order}
At first order in $\delta$, the current collector equations: (\ref{DFNCC:eqn:phi_s_cn}), (\ref{DFNCC:eqn:phi_s_cp}), (\ref{bc:nDim:reference_potential}), (\ref{bc:nDim:applied current}), and (\ref{bc:nDim:external_cc}) become
\begin{subequations}\label{eqn:first-order-current-collector}
\begin{align}
    L\ts{cn}\sigma\ts{cn}'\nabla_\perp^2 \phi\ts{s,cn}^1 = \mathcal{I}^1 \\
    L\ts{cp}\sigma\ts{cp}'\nabla_\perp^2 \phi\ts{s,cp}^1 = -\mathcal{I}^1
\end{align}
\begin{gather}
    \phi\ts{s,cn}^1 = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{tab,n}, \\
\frac{1}{L_yL_z}\int_{\partial\Omega\ts{tab,p}}\nabla_\perp\phi\ts{s,cp}^1\cdot\boldsymbol{n} = 0,\\
\nabla_\perp\phi\ts{s,k}^1\cdot\boldsymbol{n} = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{ext,k} \quad \kin{cn, cp}.
\end{gather}
\end{subequations}

The derivation of the first-order models for the electrolyte, particles, and electrode follow closely the derivation provided in \cite{Marquis2019} and so we simply provide the algebraic expressions obtained at this order in Appendix \ref{app:algebraic-expressions}. We also choose to employ the transient form of the electrolyte model; formally one should rescale time to derive this model but in this case the result is trivial, as discussed in \cite{Marquis2019}. The resulting first-order model for the lithium-ion concentration in the electrolyte is then
\begin{subequations}\label{eqn:first-order-electrolyte}
    \begin{gather}
        \mathcal{C}\ts{e} \epsilon\ts{k} \gamma\ts{e} \pdv{c\ts{e,k}^1}{t} = - \gamma\ts{e} \pdv{N\ts{e,k}^1}{x} +
        \begin{cases}
            \frac{\mathcal{I}^0}{L\ts{n}}, \quad &\text{k}=\text{n}, \\
            0, \quad &\text{k}=\text{s}, \\
            -\frac{\mathcal{I}^0}{L\ts{p}}, \quad &\text{k}=\text{p},
        \end{cases} \\
        N\ts{e,k}^1 = -\epsilon\ts{k}^{\text{b}}D\ts{e}(1, T^0)\pdv{c\ts{e,k}^1}{x}
        +
        \begin{cases}
        \frac{x t^+ \mathcal{I}^0}{\gamma\ts{e} L\ts{n}}, \quad &\text{k}=\text{n},\\
        \frac{t^+ \mathcal{I}^0}{\gamma\ts{e}}, \quad &\text{k}=\text{s},\\
        \frac{(1-x) t^+ \mathcal{I}^0}{\gamma\ts{e} L\ts{p}}, \quad &\text{k}=\text{p},
        \end{cases}\\
        c\ts{e,k}^1(x,0)=0, \quad
        N\ts{e,n}^1\big|_{x=0}=0, \quad
        N\ts{e,p}^1\big|_{x=1}=0, \\
        c\ts{e,n}^1\big|_{x=L\ts{n}}=c\ts{e,s}^1\big|_{x=L\ts{n}}, \quad
        N\ts{e,n}^1\big|_{x=L\ts{n}}=N\ts{e,s}^1\big|_{x=L\ts{n}}, \\
        c\ts{e,s}^1\big|_{x=1-L\ts{p}}=c\ts{e,p}^1\big|_{x=1-L\ts{p}}, \quad
        N\ts{e,s}^1\big|_{x=1-L\ts{p}}=N\ts{e,p}^1\big|_{x=1-L\ts{p}}.
    \end{gather}
\end{subequations}
Hence, if we need to obtain the concentration of lithium in each particle in the $x$-direction, then \eqref{eqn:first-order-electrolyte} for lithium in each particle must be solved at every location in $x$. However, as exploited in \cite{Marquis2019}, if we do not explicitly need to know the lithium concentration in detail we can solve for the concentration in a theoretical $x$-electrode-averaged particle and still obtain the potential difference across the cell correct to $\mathcal{O}(\delta^2)$. This $x$-electrode-averaged problem is given by
\begin{subequations}\label{eqn:first-order-particles}
\begin{align}
    \mathcal{C}\ts{k}\pdv{\bar{c}\ts{s,k}^1}{t} &= - \frac{1}{r\ts{k}^2}\pdv{r\ts{k}}\left(r\ts{k}^2 N^1\ts{s,k}\right),  && \kin{n, p}, \\
    N^1\ts{s,k} &= -\left(D\ts{k}(c\ts{s,k}^0, T^0)\pdv{\bar{c}\ts{s,k}^1}{r\ts{k}} + \pdv{D\ts{k}}{c\ts{s,k}} (c\ts{s,k}^0, T^0) \bar{c}\ts{s,k}^1 + \pdv{D\ts{k}}{T} (c\ts{s,k}^0, T^0) \Xav{T}^1\right), && \kin{n, p},\\
    \left.N^1\ts{s,k}\right|_{r\ts{k}=0} &= 0, \quad
     \frac{a\ts{k}\gamma\ts{k}}{\mathcal{C}\ts{k}}\left.N^1\ts{s,k} \right|_{r\ts{k}=1} =
     \begin{cases}
     \frac{\mathcal{I}^1}{L\ts{n}}, \quad & \text{k} = \text{n}, \\
     -\frac{\mathcal{I}^1}{L\ts{p}}, \quad & \text{k} = \text{p},
     \end{cases}, && \kin{n, p},\\
     \bar{c}\ts{s,k}^1(r,y,z,0) &= 0, && \kin{n, p},
\end{align}
\end{subequations}
To be consistent when employing the solution to the $x$-electrode-averaged PDE problem in the particles, we also need to express the other variables at first order in $x$-electrode-averaged form. The expressions for these terms are provided in Appendix \ref{app:electrode_averaged}.

Finally, at first order in $\delta$, the thermal problem (\ref{DFNCC:eqn:thermal}), (\ref{DFNCC:BC:tempext}), and (\ref{ic:nDim:temp}) becomes
\begin{subequations}\label{eqn:first-order-temperature}
\begin{align}
    \mathcal{C}\ts{th} \rho \pdv{T^1}{t} &= \lambda \nabla_\perp^2T^1 + \mathcal{B}\bar{Q}^1 - \frac{2h'}{L}T^1, \\
     -\lambda \nabla_\perp {T^1} \cdot \boldsymbol{n} &= h' T^0, && (y,z) \in \partial\Omega\ts{ext}, \\
     T^1\big\vert_{t=0} &= 0, &&
     \end{align}
\end{subequations}
where the heat generation term, $\bar{Q}^1$, is provided in Appendix~\ref{app:heatgen}.

\subsubsection{Combined leading- and first-order model: 2+1D SPMe}\label{sec:2p1-SPMe}
Whilst Sections \ref{sec:2p1-SPM} and \ref{sec:poor-cc-first-order} contain all of the components required to solve the leading- and first-order models, it is convenient to combine the leading- and first-order models for the purposes of both implementation and interpretation. We employ the notation of a superscript `c' to indicate combined-order terms, defined by
\begin{equation*}
    c\ts{s,k}\co := c\ts{s,k}^0 + \delta c\ts{s,k}^1
\end{equation*}
for each of the variables, and we also make use of the fact that the $x$-electrode-averages are then in the form 
\begin{equation*}
    \Xav{c}\ts{s,k}\co = c\ts{s,k}^0 + \delta \Xav{c}\ts{s,k}^1.
\end{equation*}

Combining \eqref{eqn:leading-order-current-collector} and \eqref{eqn:first-order-current-collector}, we obtain the following combined problem for the current collector potentials,
\begin{subequations}\label{eqn:combined-current-collector}
    \begin{align}
        L\ts{cn}\sigma\ts{cn}'\nabla_\perp^2 \phi\ts{s,cn}\co = \mathcal{I}\co \\
        L\ts{cp}\sigma\ts{cp}'\nabla_\perp^2 \phi\ts{s,cp}\co = -\mathcal{I}\co
    \end{align}
    \begin{gather}
        \phi\ts{s,cn}\co = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{tab,n}, \\
    \frac{1}{L_yL_z}\int_{\partial\Omega\ts{tab,p}}\nabla_\perp\phi\ts{s,cp}\co\cdot\boldsymbol{n} = - \frac{I_{\text{app}}}{\sigma\ts{cp}'}\\
    \nabla_\perp\phi\ts{s,k}\co\cdot\boldsymbol{n} = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{ext,k} \quad \kin{cn, cp}.
    \end{gather}
\end{subequations}

The leading-order solution in the electrolyte is simply $c\ts{e,k}=1$. It is simple to incorporate this leading-order solution into the first-order electrolyte problem \eqref{eqn:first-order-electrolyte}. However, in the combined problem, we do not find $\mathcal{I}^0$ as part of the solution. Therefore, the terms involving $\mathcal{I}^0$ in \eqref{eqn:first-order-electrolyte} are unknown. Fortunately, since $\mathcal{I}^0$ only appears in the $\mathcal{O}(\delta)$ equations and $\delta\mathcal{I}^0 = \delta\mathcal{I}\co + \mathcal{O}(\delta^2)$, we can replace $\mathcal{I}^0$ by $\mathcal{I}\co$ and still retain $\mathcal{O}(\delta^2)$ accuracy. A similar argument holds for replacing $D\ts{e}(1,T^0)$ by $D\ts{e}(c\ts{e,k}\co, T\co)$. The resulting combined-order problem is then given by
\begin{subequations}\label{eqn:combined-electrolyte}
    \begin{gather}
        \mathcal{C}\ts{e} \epsilon\ts{k} \gamma\ts{e} \pdv{c\ts{e,k}\co}{t} = - \gamma\ts{e} \pdv{N\ts{e,k}\co}{x} +
        \mathcal{C}\ts{e}
        \begin{cases}
            \frac{\mathcal{I}\co}{L\ts{n}}, \quad &\text{k}=\text{n}, \\
            0, \quad &\text{k}=\text{s}, \\
            -\frac{\mathcal{I}\co}{L\ts{p}}, \quad &\text{k}=\text{p},
        \end{cases} \\
        N\ts{e,k}\co = -\epsilon\ts{k}^{\text{b}}D\ts{e}(c\ts{e,k}\co, T\co)\pdv{c\ts{e,k}\co}{x} +
        \mathcal{C}\ts{e}
        \begin{cases}
        \frac{x t^+ \mathcal{I}\co}{\gamma\ts{e} L\ts{n}}, \quad &\text{k}=\text{n},\\
        \frac{t^+ \mathcal{I}\co}{\gamma\ts{e}}, \quad &\text{k}=\text{s},\\
        \frac{(1-x) t^+ \mathcal{I}\co}{\gamma\ts{e} L\ts{p}}, \quad &\text{k}=\text{p},
        \end{cases}\\
        c\ts{e,k}\co(x,0)=1, \quad
        N\ts{e,n}\co\big|_{x=0}=0, \quad
        N\ts{e,p}\co\big|_{x=1}=0, \\
        c\ts{e,n}\co\big|_{x=L\ts{n}}=c\ts{e,s}\co\big|_{x=L\ts{n}}, \quad
        N\ts{e,n}\co\big|_{x=L\ts{n}}=N\ts{e,s}\co\big|_{x=L\ts{n}}, \\
        c\ts{e,s}\co\big|_{x=1-L\ts{p}}=c\ts{e,p}\co\big|_{x=1-L\ts{p}}, \quad
        N\ts{e,s}\co\big|_{x=1-L\ts{p}}=N\ts{e,p}\co\big|_{x=1-L\ts{p}}.
    \end{gather}
\end{subequations}

To combine the particle equations so that we have a combined-order model for the $x$-electrode-averaged particle, we first note that the leading-order lithium concentration in the particles is independent of $x$ and so $\Xav{c}\ts{s,k}^0=c\ts{s,k}^0$. Then combining \eqref{eqn:leading-order-particles} and \eqref{eqn:first-order-particles} by re-combining the first two terms of the Taylor expansion yields a combined model that is accurate $\mathcal{O}(\delta^2)$ given by
\begin{subequations}\label{eqn:combined-order-particles}
    \begin{gather}
         \mathcal{C}\ts{k}\pdv{\Xav{c}\ts{s,k}\co}{t} = -\frac{1}{r\ts{k}^2}\pdv{r\ts{k}}
            \left(
                r\ts{k}^2 D\ts{k}(\Xav{c}\ts{s,k}\co, T\co)
                \pdv{\Xav{c}\ts{s,k}\co}{r\ts{k}}
            \right), \quad \kin{n, p} \\
        \pdv{\Xav{c}\ts{s,k}\co}{r\ts{k}}\bigg|_{r\ts{k}=0}=0, \quad
        -\frac{a\ts{k}\gamma\ts{k}}{\mathcal{C}\ts{k}}
            D\ts{k}(\Xav{c}\ts{s,k}\co, T\co)
            \pdv{\Xav{c}\ts{s,k}\co}{r\ts{k}}\bigg|_{r\ts{k}=0}=,
         \begin{cases}
         \frac{\mathcal{I}\co}{L\ts{n}}, \quad & \text{k}=\text{n}, \\
         -\frac{\mathcal{I}\co}{L\ts{p}}, \quad &\text{k}=\text{p},
         \end{cases} \label{eqn:lo:solidConcentration:BC} \\
         \Xav{c}\ts{s,k}\co(r\ts{k},0) = c\ts{s,k,0}, \quad \kin{n, p}.
    \end{gather}
\end{subequations}

Combining the thermal problems \eqref{eqn:leading-order-temperature} and \eqref{eqn:first-order-temperature} gives
\begin{subequations}\label{eqn:combined-order-temperature}
    \begin{gather}
        \mathcal{C}\ts{th} \rho \pdv{T\co}{t} = \lambda \nabla_\perp^2T\co + \mathcal{B}\bar{Q}\co - \frac{2 h'}{L} T\co,    \\
        - \lambda \nabla_\perp T\co \cdot \boldsymbol{n} = \delta h' T\co, \quad T\co(y,z,0) =T_0
    \end{gather}
\end{subequations}
where $Q\co$ is provided in Appendix \ref{app:heatgen}.


To complete the problem in a simple form, it is useful to express $\phi\ts{s,cp}$ in terms of $\phi\ts{s,cn}$ and the 1D through-cell internal states. By combing the leading- and first-order terms from Appendix \ref{app:algebraic-expressions} and \ref{app:electrode_averaged}, we obtain
\begin{subequations}\label{eqn:combined-order-potential-difference}
\begin{align}
    \phi\ts{s,cp}\co &= \phi\ts{s,cn}\co + \Xav{U}\ts{eq}\co + \Xav{\eta}\ts{r}\co + \Xav{\eta}\ts{c}\co + \Xav{\Delta\Phi}\ts{Elec}\co + \Xav{\Delta\Phi}\ts{Solid}\co
\end{align}
where
\begin{align}
    &\Xav{U}\ts{eq}\co = U\ts{p}(\Xav{c}\ts{s,p}\co, T\co) - U\ts{n}(\Xav{c}\ts{s,n}\co, T\co), \\
    &\Xav{\eta}\ts{r}\co = \Xav{\eta}\ts{p}\co - \Xav{\eta}\ts{n}\co, \\
    &\Xav{\eta}\ts{k}\co = 2 (1 + \Theta T\co) \sinh^{-1}\left(\frac{\Xav{j}\ts{k}\co}{\Xav{j}\ts{0,k}\co}\right) \quad\kin{n, p},\\
    &\Xav{j}\ts{n}\co = \frac{\mathcal{I}\co}{L\ts{n}},\\
    &\Xav{j}\ts{p}\co = -\frac{\mathcal{I}\co}{L\ts{p}}, \\
    &\Xav{j}\ts{0,k}\co = \frac{\gamma\ts{k}}{\mathcal{C}\ts{r,k}}m\ts{k}(T\co) (\Xav{c}\ts{s,k}\co)^{1/2}  (1 - \Xav{c}\ts{s,k}\co)^{1/2}(\Xav{c}\ts{e,k}\co)^{1/2}, \\
    &\Xav{\eta}\ts{c}\co = 2(1-t^+)(\Xav{c}\ts{e,p}\co-\Xav{c}\ts{e,n}\co),\\
    &\Xav{\Delta\Phi}\ts{Elec} = - \frac{\mathcal{I}\co}{\hat{\kappa}\kappa\ts{e}(1)}\left(\frac{L\ts{n}}{3\epsilon\ts{n}^b} + \frac{L\ts{s}}{\epsilon\ts{s}^b} + \frac{L\ts{p}}{3\epsilon\ts{p}^b} \right), \\
    &\Xav{\Delta\Phi}\ts{Solid} = -\frac{\mathcal{I}\co}{3}\left(\frac{L\ts{p}}{\sigma\ts{p}} + \frac{L\ts{n}}{\sigma\ts{n}} \right),
\end{align}
where we have again made use of the fact that $\mathcal{I}^0$ can be replaced by $\mathcal{I}\co$ in the first-order expression with $\mathcal{O}(\delta^2)$ accuracy being retained.
% scott: I think we only need a delta in here (and not a C_e as in 1D case) because we expand c_e in powers of delta instead of C_e and so C_e' is contained in c_e^1 and so also c_e^c.
\end{subequations}

The system: \eqref{eqn:combined-current-collector}, \eqref{eqn:combined-electrolyte}, \eqref{eqn:combined-order-particles}, \eqref{eqn:combined-order-temperature}, and \eqref{eqn:combined-order-potential-difference} now forms a closed system of equations which can be solved numerically. The model consists of two 2D current collector problems coupled to a 1D SPMe at every $(y,z)$ point and also coupled to a 2D thermal problem. We shall therefore refer to this combined-order model as the 2+1D SPMe.

At the next order the potential difference must satisfy
\begin{equation}\label{eqn:asim:V1poisson}
    \nabla_\perp^2\mathcal{V}^1 = -\alpha \mathcal{I}^1,
\end{equation}
with $\nabla_\perp\mathcal{V}^1\cdot\boldsymbol{n} = 0$ on the boundary. At $\mathcal{O}(\delta)$, \eqref{eqn:nDim:electrolyte:concentration} and \eqref{eqn:nDim:electrolyte:flux} give
\begin{equation}\label{eqn:od:flux}
    \gamma\ts{e}\pdv{N\ts{e,k}^1}{x} = \mathcal{C}\ts{e}' \pdv{i\ts{e,k}^0}{x}, \quad
    N\ts{e,k}^1 = -\epsilon\ts{k}^{\text{b}} D\ts{e}(c^0\ts{e,k}, T^0) \pdv{c^1\ts{e,k}}{x} + \frac{\mathcal{C}\ts{e}' t^+}{\gamma\ts{e}}i\ts{e,k}^0, \quad  \kin{n, p}.
\end{equation}
The dependence on the concentration may be removed by integration of \eqref{eqn:od:flux}$_1$ over region $\Omega\ts{k}$ for $\kin{n, s, p}$, giving
\begin{equation}\label{eqn:od:fluxes:sol}
    N\ts{e,n}^1 = \frac{\mathcal{C}\ts{e}'}{\gamma\ts{e}}\frac{ \mathcal{I}^0 x}{L\ts{n}}, \quad N\ts{e,s} = \frac{\mathcal{C}\ts{e}'}{\gamma\ts{e}} \mathcal{I}^0, \quad N\ts{e,p}^1 = \frac{\mathcal{C}\ts{e}'}{\gamma\ts{e}}\frac{ \mathcal{I}^0 (1-x)}{L\ts{p}}.
\end{equation}
Substitution of \eqref{eqn:od:fluxes:sol} into \eqref{eqn:od:flux} and integrating with respect to $x$ over $\Omega\ts{k}$ for $\kin{n, s, p}$ gives the corrections to the lithium-ion concentration in the electrolyte
\begin{subequations}
\begin{align}
    &c\ts{e,n}^1 = \frac{\mathcal{C}\ts{e}'}{\gamma\ts{e}}\frac{(1-t^+) \mathcal{I}^0}{ 6 D(1, T^0)}
        \left( 2\left(\frac{L\ts{p}^2}{\epsilon\ts{p}^{\text{b}}} - \frac{L\ts{n}^2}{\epsilon\ts{n}^{\text{b}}}\right)
         +\frac{3L\ts{s}}{\epsilon\ts{s}^{\text{b}}}(1+L\ts{p}-L\ts{n}) + \frac{3}{\epsilon\ts{n}^{\text{b}} L\ts{n}}(L\ts{n}^2-x^2)
         \right), \\
    &c\ts{e,s}^1 = \frac{\mathcal{C}\ts{e}'}{\gamma\ts{e}}\frac{(1-t^+) \mathcal{I}^0}{ 6 D(1, T^0)}
        \left( 2\left(\frac{L\ts{p}^2}{\epsilon\ts{p}^{\text{b}}} - \frac{L\ts{n}^2}{\epsilon\ts{n}^{\text{b}}}\right)
         +\frac{3}{\epsilon\ts{s}^{\text{b}}}(L\ts{n}^2 - L\ts{p}^2 + 1-2x)
         \right), \\
    &c\ts{e,p}^1 = \frac{\mathcal{C}\ts{e}'}{\gamma\ts{e}}\frac{(1-t^+) \mathcal{I}^0}{ 6 D(1, T^0)}
        \left( 2\left(\frac{L\ts{p}^2}{\epsilon\ts{p}^{\text{b}}} - \frac{L\ts{n}^2}{\epsilon\ts{n}^{\text{b}}}\right)
         +\frac{3L\ts{s}}{\epsilon\ts{s}^{\text{b}}}(L\ts{p} - L\ts{n} - 1) + \frac{3}{L\ts{p} \epsilon\ts{p}^{\text{b}}}( (x-1)^2 - L\ts{p}^2 )
         \right),
\end{align}
\end{subequations}
where we have used the $\mathcal{O}(\delta)$ components of the boundary conditions \eqref{bc:nDim:concentration_continuity_Ln} and \eqref{bc:nDim:concentration_continuity_Lp}, and conservation of lithium to determine the constants of integration.

At $\mathcal{O}(\delta)$, \eqref{eqn:nDim:McIn} reads
\begin{gather}\label{eqn:od:current_to_integrate}
        \mathcal{C}\ts{e}'i\ts{e,k}^0 = \epsilon\ts{k}^{\text{b}} \kappa'\ts{e}\kappa\ts{e}(1, T^0) \left( - \pdv{\phi^1\ts{e,k}}{x} + 2(1-t^+)(1 + \Theta T^0)\pdv{c\ts{e,k}^1}{x} \right).
\end{gather}
Substituting \eqref{eqn:lo:current} into \eqref{eqn:od:current_to_integrate} and integrating with respect to $x$ over $\Omega\ts{k}$ for $\kin{n, s, p}$  provides the corrections to the electrical potential in the electrolyte
\begin{subequations}
    \begin{align}
        &\phi\ts{e,n}^1 = \hat{\phi}\ts{e} + 2(1-t^+)(1 + \Theta T^0)c\ts{e,n}^1
        - \frac{\mathcal{C}\ts{e}'\mathcal{I}^0}{\kappa'\ts{e} \kappa\ts{e}(1, T^0)}\left(\frac{x^2-L\ts{n}^2}{2 \epsilon\ts{n}^{\text{b}} L\ts{n}} + \frac{L\ts{n}}{\epsilon\ts{s}^{\text{b}}} \right), \\
         &\phi\ts{e,s}^1 = \hat{\phi}\ts{e}  + 2(1-t^+) (1 + \Theta T^0)c\ts{e,s}^1
        - \frac{\mathcal{C}\ts{e}' \mathcal{I}^0 x}{\kappa'\ts{e} \kappa\ts{e}(1, T^0)\epsilon\ts{s}^{\text{b}}},\\
        &\phi\ts{e,n}^1 = \hat{\phi}\ts{e} + 2(1-t^+) (1 + \Theta T^0)c\ts{e,p}^1
        - \frac{\mathcal{C}\ts{e}' \mathcal{I}^0}{\kappa'\ts{e} \kappa\ts{e}(1, T^0)}\left(\frac{x(2-x)+L\ts{p}^2-1}{2\epsilon\ts{p}^{\text{b}} L\ts{p}} + \frac{1-L\ts{p}}{\epsilon\ts{s}^{\text{b}}} \right),
    \end{align}
\end{subequations}
where two of the three constants of integration have been determined by applying the $\mathcal{O}(\delta)$ components of the interior boundary conditions \eqref{bc:nDim:charge_continuity_Ln} and \eqref{bc:nDim:concentration_continuity_Lp}, and $\hat{\phi}_e$ remains as an as-yet undetermined constant. To determine the electrical potentials in the solid we consider the $\mathcal{O}(\delta)$ terms in \eqref{eqn:nDim:solid:ohms}, which read
\begin{equation}
    \mathcal{I}^0 - i\ts{e,k}^0 = -\sigma\ts{k}' \pdv{\phi\ts{s,k}^1}{x}, \quad \kin{n, p},
\end{equation}
and may be integrated with respect to $x$ to give
\begin{subequations} \label{eqn:phisolid1}
\begin{align}
    &\phi\ts{s,n}^1 = \phi\ts{s,n}^1 \big|_{x=0} + \frac{\mathcal{I}^0x}{2\sigma\ts{n}' L\ts{n}}\left(2L\ts{n} - x\right), \\
    &\phi\ts{s,p}^1 = \phi\ts{s,p}^1 \big|_{x=1} +   \frac{\mathcal{I}^0 (x-1) (1-2L\ts{p}-x)}{2\sigma\ts{p}' L\ts{p}},
\end{align}
\end{subequations}
where we have used \eqref{eqn:lo:current} to evaluate the leading-order electrolyte current.

The $\mathcal{O}(\delta)$ components of \eqref{eqn:nDim:BV}--\eqref{eqn:nDim:exchange_current} are readily computed to be

where $\eta\ts{k}^0$ and $j\ts{0,k}^0$ are given by \eqref{eqn:lo:eta} and \eqref{eqn:lo:exchange_current}, respectively. We now integrate \eqref{eqn:od:all_BV} in $x$ over $\Omega\ts{k}$ for $\kin{n, p}$, and rearrange to obtain to $x$-averaged electrical potentials in the electrodes
\begin{align}
    \nonumber
    \bar{\phi}\ts{s,n}^1 &=  \bar{\phi}\ts{e,n}^1 +  \pdv{U\ts{n}}{c\ts{s,n}} (c\ts{s,n}^0,T^0) \bar{c}\ts{n}^1 + \pdv{U\ts{n}}{T} (c\ts{s,n}^0,T^0)T^1 \\
    \label{eqn:od:av_phi_n}
    &\quad + \frac{2 \mathcal{I}^1}{j\ts{0,n}^0 L\ts{n}}\sech\left(\frac{\eta\ts{n}^0}{2(1 + \Theta T^0)}\right) - \frac{2 \bar{j}\ts{0,n}^1}{j\ts{0,n}^0 L\ts{n}}\tanh{\left(\frac{\eta\ts{n}^0}{2(1 + \Theta T^0)}\right)} + \frac{\Theta T^1}{1 + \Theta T^0}, \\
    \nonumber
    \bar{\phi}\ts{s,p} &= \bar{\phi}\ts{e,p}^1 + \pdv{U\ts{p}}{c\ts{s,p}} (c\ts{s,p}^0,T^0) \bar{c}\ts{s,p}^1 + \pdv{U\ts{p}}{T} (c\ts{s,p}^0,T^0)T^1 \\
    \label{eqn:of:av_phi_p}
    &\quad - \frac{2 \mathcal{I}^1}{j\ts{0,p}^0 L\ts{p}}\sech\left(\frac{\eta\ts{p}^0}{2(1 + \Theta T^0)}\right) - \frac{2 \bar{j}\ts{0,p}^1}{j\ts{0,p}^0 L\ts{p}}\tanh{\left(\frac{\eta\ts{p}^0}{2(1 + \Theta T^0)}\right)} + \frac{\Theta T^1}{1 + \Theta T^0},
\end{align}
where we have averaged the $\mathcal{O}(\delta)$ component of \eqref{eqn:nDim:electrolyte:current} over each electrode, and applied the boundary conditions \eqref{bc:nDim:no_electrolyte_cc_current}--\eqref{bc:nDim:charge_continuity_Lp} to give the $x$-averaged corrections to the reaction flux densities
\begin{equation}\label{eqn:od:conditions}
	\bar{j}\ts{n}^1 = \frac{1}{L\ts{n}}\int_0^{L\ts{n}} j\ts{n}^1 \dd{x} = \frac{\mathcal{I}^1}{L\ts{n}}, \ \ 	\bar{j}\ts{p}^1 = \frac{1}{L\ts{p}}\int_{1-L\ts{p}}^1 j\ts{p}^1 \dd{x} = - \frac{\mathcal{I}^1}{L\ts{p}}.
\end{equation}


Now, we may calculate the correction to the potential difference by averaging \eqref{eqn:phisolid1} over each electrode, the result being
\begin{subequations} \label{eqn:phisolid1av}
\begin{align}
    &\bar{\phi}\ts{s,n}^1 = \frac{1}{L\ts{n}}\int_0^{L\ts{n}} \phi\ts{s,n}^1 \dd{x} = \phi\ts{s,n}^1 \big|_{x=0} - \frac{\mathcal{I}^0L\ts{n}}{3\sigma\ts{n}'}, \\
    &\bar{\phi}\ts{s,p}^1 = \frac{1}{L\ts{p}}\int_{1-L\ts{p}}^1 \phi\ts{s,p}^1 \dd{x} = \phi\ts{s,p}^1 \big|_{x=1} +\frac{\mathcal{I}^0L\ts{p}}{3\sigma\ts{p}'},
\end{align}
\end{subequations}
which gives
\begin{equation}\label{eqn:asim1:V1}
    \begin{split}
        \mathcal{V}^1 &= \phi\ts{s,p}^1\big\vert_{x=1} - \phi\ts{s,n}^1\big\vert_{x=0}  \\
    &= \bar{\phi}\ts{s,p}^1 - \bar{\phi}\ts{s,n}^1 - \frac{\mathcal{I}^0}{3}\left( \frac{L\ts{p}}{\sigma\ts{p}'} + \frac{L\ts{n}}{\sigma\ts{n}'}\right) \\
    &= \bar{\phi}\ts{e,p}^1 - \bar{\phi}\ts{e,n}^1 - \frac{2 \mathcal{I}^1}{j\ts{0,p}^0 L\ts{p}}\sech\left(\frac{\eta\ts{p}^0}{2(1 + \Theta T^0)}\right) - \frac{2 \mathcal{I}^1}{j\ts{0,n}^0 L\ts{n}}\sech\left(\frac{\eta\ts{n}^0}{2(1 + \Theta T^0)}\right) \\
    &\quad - \frac{2 \bar{j}\ts{0,p}^1}{j\ts{0,p}^0 L\ts{p}}\tanh{\left(\frac{\eta\ts{p}^0}{2(1 + \Theta T^0)}\right)} + \frac{2 \bar{j}\ts{0,n}^1}{j\ts{0,n}^0 L\ts{n}}\tanh{\left(\frac{\eta\ts{n}^0}{2(1 + \Theta T^0)}\right)} \\
    &\quad + \pdv{U\ts{p}}{c\ts{s,p}} (c\ts{s,p}^0,T^0) \bar{c}\ts{s,p}^1 + \pdv{U\ts{p}}{T} (c\ts{s,p}^0,T^0)T^1 - \pdv{U\ts{n}}{c\ts{s,n}} (c\ts{s,n}^0,T^0) \bar{c}\ts{s,n}^1 - \pdv{U\ts{n}}{T} (c\ts{s,n}^0,T^0)T^1 \\
    &\quad - \frac{\mathcal{I}^0}{3}\left( \frac{L\ts{p}}{\sigma\ts{p}'} + \frac{L\ts{n}}{\sigma\ts{n}'}\right).
    \end{split}
\end{equation}
\rob{Scott, I think you had a nicer way of writing this as in your SPMe paper in terms of square roots etc Would be nice to be able to interpret physically here, and compare extra terms which arise from 2D and thermal effects}

This must then be solved in conjunction with the problem relating the potential difference and current \eqref{eqn:asim:V1poisson}, the problem for the $x$-averaged correction to the particle concentration
\begin{subequations}\label{eqn:od:electrode_av_con}
\begin{align}
    \mathcal{C}\ts{k}\pdv{\bar{c}\ts{s,k}^1}{t} &= - \frac{1}{r\ts{k}^2}\pdv{r\ts{k}}\left(r\ts{k}^2 N^1\ts{s,k}\right),  && \kin{n, p}, \\
    N^1\ts{s,k} &= -\left(D\ts{k}(c\ts{s,k}^0, T^0)\pdv{\bar{c}\ts{s,k}^1}{r\ts{k}} + \pdv{D\ts{k}}{c\ts{s,k}} (c\ts{s,k}^0, T^0) \bar{c}\ts{s,k}^1 + \pdv{D\ts{k}}{T} (c\ts{s,k}^0, T^0) T^1\right), && \kin{n, p},\\
    \left.N^1\ts{s,k}\right|_{r\ts{k}=0} &= 0, \quad
     \frac{a\ts{k}\gamma\ts{k}}{\mathcal{C}\ts{k}}\left.N^1\ts{s,k} \right|_{r\ts{k}=1} =
     \begin{cases}
     \frac{\mathcal{I}^1}{L\ts{n}}, \quad & \text{k} = \text{n}, \\
     -\frac{\mathcal{I}^1}{L\ts{p}}, \quad & \text{k} = \text{p},
     \end{cases}, && \kin{n, p},\\
     \bar{c}\ts{s,k}^1(r,y,z,0) &= 0, && \kin{n, p},
\end{align}
\end{subequations}
\end{comment}

\begin{comment}
\subsection{High current collector conductance}\label{sec:high-cc}
In this section, we take the limit of high current collector conductance, that is we take the typical potential drop in the current collector to be much smaller than the thermal voltage.
In particular, we consider $\delta \to 0$ with
\begin{equation}\label{eqn:highly-conducting-current-collectors}
    \sigma\ts{cn}' = \frac{\sigma\ts{cn}''}{\delta} =\mathcal{O}\left(\frac{1}{\delta}\right),\qquad
    \sigma\ts{cp}' = \frac{\sigma\ts{cp}''}{\delta} =\mathcal{O}\left(\frac{1}{\delta}\right),
\end{equation}
whilst taking all other parameters in \eqref{DFNCC} to be $\mathcal{O}(1)$ and then
expand all variables in powers of $\delta$ as in \eqref{eqn:expand}.

\subsubsection{Leading-order model: 1D DFN}
At leading-order in $\delta$, the current collector problem: (\ref{DFNCC:eqn:phi_s_cn}), (\ref{DFNCC:eqn:phi_s_cp}), (\ref{bc:nDim:reference_potential}), (\ref{bc:nDim:applied current}), and (\ref{bc:nDim:external_cc}) becomes
\begin{subequations}\label{eqn:high-cc:leading-order-current-collector}
    \begin{align}
        L\ts{cn}\sigma\ts{cn}''\nabla_\perp^2 \phi\ts{s,cn}^0 = 0 \\
        L\ts{cp}\sigma\ts{cp}''\nabla_\perp^2 \phi\ts{s,cp}^0 = 0
    \end{align}
    \begin{gather}
        \phi\ts{s,cn}^0 = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{tab,n}, \\
    \frac{1}{L_yL_z}\int_{\partial\Omega\ts{tab,p}}\nabla_\perp\phi\ts{s,cp}^0\cdot\boldsymbol{n} = 0\\
    \nabla_\perp\phi\ts{s,k}^0\cdot\boldsymbol{n} = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{ext,k} \quad \kin{cn, cp}.
    \end{gather}
\end{subequations}
Hence the leading-order potential in the negative current collector is simply $\phi\ts{s,cn}^0=0$ and the leading-order potential in the positive current collector $\phi\ts{s,cp}^0$ is spatially independent, with the constant of integration determined by the condition $\phi\ts{s,n}^0\big|_{x=1}=V^0$ (i.e. the leading-order terminal voltage). By considering the $\mathcal{O}(\delta)$ current collector equations and the fact that the leading-order internal cell problem is initially independent of $y$ and $z$, it can be shown that the leading-order current is given by
\begin{equation}
    \mathcal{I}^0 = I\ts{app}
\end{equation}
which is equivalent to the average (across all 1D models) current density entering the 1D models in \eqref{DFNCC}. Since this leading-order current density is independent of $y$ and $z$, and since the initial conditions considered here are independent of $y$ and $z$, each of the 1D electrochemical models behaves in exactly the same way. Therefore, it is sufficient to solve for a single representative 1D DFN model in the through-cell direction. In the isothermal case, this leading-order model is then just the original 1D DFN model first developed by Newman and collaborators \cite{doyle1993}.

In this limit, at leading-order the thermal model (\ref{DFNCC:eqn:thermal}), (\ref{DFNCC:BC:tempext}), and (\ref{ic:nDim:temp}) reduces to
\begin{subequations}\label{eqn:high-cc:leading-order-thermal}
\begin{gather}
\frac{\rho}{\gamma\ts{th}} \dv{T^0}{t} =  \mathcal{B}\bar{Q}^0 - \frac{2 h'}{L} T^0, \\
T^0(0) = T_0
\end{gather}
\end{subequations}
where the leading-order heat generation is given by the expressions in Appendix \ref{app:high-no-diff}. Note that the boundary condition \eqref{DFNCC:BC:tempext} appears at $\mathcal{O}(\delta)$, that is, the heat transfer coefficient is sufficiently small so that only surface cooling on the faces of the pouch cell is significant to leading-order. We refer to this model as the 1D DFN model.

\subsubsection{Combined leading- and first-order model: DFNCC}\label{sec:DFNCC}
By proceeding to $\mathcal{O}(\delta)$, we can improve the 1D DFN model at the expense of performing a once-and-for-all initial solve of the current collector problem. At this order, the current collector problem reduces to
\begin{subequations}\label{eqn:high-cc:first-order-current-collector}
    \begin{align}
        L\ts{cn}\sigma\ts{cn}''\nabla_\perp^2 \phi\ts{s,cn}^1 =I\ts{app}\\
        L\ts{cp}\sigma\ts{cp}''\nabla_\perp^2 \phi\ts{s,cp}^1 = -I\ts{app}
    \end{align}
    \begin{gather}
        \phi\ts{s,cn}^1 = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{tab,n}, \\
    \frac{1}{L_yL_z}\int_{\partial\Omega\ts{tab,p}}\nabla_\perp\phi\ts{s,cp}^1\cdot\boldsymbol{n} = 0\\
    \nabla_\perp\phi\ts{s,k}^1\cdot\boldsymbol{n} = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{ext,k} \quad \kin{cn, cp}.
    \end{gather}
\end{subequations}
This problem is dependent upon the applied current which is in general a function of time. However, we can reformulate the current collector problem in terms of the current collector resistances, which we define to be
\begin{equation}\label{eqn:high-cc:potentials}
    R\ts{cn} := \frac{\phi\ts{s,cn}}{I\ts{app}}, \quad R\ts{cp} := \frac{V - \phi\ts{s,cp}}{I\ts{app}},
\end{equation}
where $V$ is the terminal voltage. We refer to these terms as resistances despite them being negative when the current is negative; we have chosen to do this to simplify notation. Upon making this change of variables, the combined leading- and first-order problem in the resistors becomes
\begin{subequations}\label{eqn:high-cc:combined-order-current-collector}
    \begin{align}
        L\ts{cn}\sigma\ts{cn}''\nabla_\perp^2 R\ts{cn}\co = \delta \\
        L\ts{cp}\sigma\ts{cp}''\nabla_\perp^2 R\ts{cp}\co = \delta
    \end{align}
    \begin{gather}
        R\ts{cn}\co = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{tab,n}, \\
        R\ts{cp}\co = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{tab,p}, \\
    \nabla_\perp R\ts{k}\co\cdot\boldsymbol{n} = 0, \quad \boldsymbol{x} \in \partial \Omega\ts{ext,k} \quad \kin{cn, cp},
    \end{gather}
\end{subequations}
which can be solved once-and-for-all (i.e. independent of time) for a particular geometry. We note that one could rescale $R\ts{cn}\co$ and $R\ts{cp}$ to make \eqref{eqn:high-cc:combined-order-current-collector} independent of all of the dimensionless parameters in the model and convert it into a purely geometric problem. However, we have not done so here to maintain the simple physical interpretation of solving the problem for the resistance. It should be noted that numerically it is beneficial to solve either the first-order problem for the resistance or a problem where the small parameter, $\delta$, has been scaled out.

So far, we can determine $\phi\ts{s,cn}\co$ but we only know $\phi\ts{s,cp}\co$ up to the terminal voltage, $V$. To find $V$, we write the terminal voltage in the  $y$-$z$ averaged form given by
\begin{equation}\label{eqn:y-z-voltage}
    V = \YZav{\phi}\ts{s,cn}\co + \left(V-\YZav{\phi}\ts{s,cp}\co\right) + \left(\YZav{\phi}\ts{s,cp}\co - \YZav{\phi}\ts{s,cn}\co\right).
\end{equation}
The first two terms: $\YZav{\phi}\ts{s,cn}\co$ and $\left(V-\YZav{\phi}\ts{s,cp}\co\right)$ are determined exactly by solving \eqref{eqn:high-cc:combined-order-current-collector}. Therefore it only remains to determine the final term. This term represents $y-z$-averaged current collector to current collector potential difference. It can be seen by an argument of conservation of current that $\YZav{\mathcal{I}^1}=0$. Therefore upon $y$-$z$-averaging the combined leading- and first-order 1D DFN models, we obtain a problem for a single 1D DFN model with an input current of$I\ts{app}$, which is the same 1D problem that we had to solve at leading order. At combined leading- and first-order the thermal problem (\ref{DFNCC:eqn:thermal}), (\ref{DFNCC:BC:tempext}), and (\ref{ic:nDim:temp}) becomes the same as that stated in \eqref{eqn:combined-order-temperature} but with the heating term given by the expression in Appendix \ref{app:high-no-diff}. At leading-order we only had to solve for a single representative 1D DFN because all 1D electrochemical models behaved in exactly the same way. In contrast, here we still solve only a single 1D DFN, but this is a theoretical $y-z$-averaged 1D DFN model which does not necessarily represent the behaviour at any particular $y-z$ point. We refer to this model as the DFNCC where the `CC' represents the decoupled current collector problem which is to be solved alongside the standard 1D DFN model.

% \scott{Using the DFNCC terminal voltage, we can work out the potentials on the current collectors and use those as inputs to a set of potentiostatic 1D DFN problems which will allow us to obtain the concentration profiles, and first-order current... Should we mention this?}

\subsection{Fast electrolyte diffusion with highly conducting electrodes and electrolyte, and high current collector conductance}\label{sec:combined-limits}
We now consider the limit of `high current collector conductance' in conjunction with 'fast electrolyte diffusion and highly conduction electrodes and electrolyte'. Mathematically, this corresponds to taking $\delta \to 0$ with 
\begin{gather}\label{eqn:highly-conducting-with-fast-diffusion}
    \begin{split}
        \mathcal{C}\ts{e}=\delta \mathcal{C}\ts{e}'=\mathcal{\delta}, \quad
            \sigma\ts{cn}' = \frac{\sigma\ts{cn}''}{\delta} =\mathcal{O}\left(\frac{1}{\delta}\right),\qquad
    \sigma\ts{cp}' = \frac{\sigma\ts{cp}''}{\delta} =\mathcal{O}\left(\frac{1}{\delta}\right),\\
               \sigma\ts{n}' = \frac{\sigma\ts{n}''}{\delta} =\mathcal{O}\left(\frac{1}{\delta}\right),\qquad
    \sigma\ts{p}' = \frac{\sigma\ts{p}''}{\delta} =\mathcal{O}\left(\frac{1}{\delta}\right),
        \hat{\kappa}\ts{e}' = \frac{\hat{\kappa}\ts{e}''}{\delta} =\mathcal{O}\left(\frac{1}{\delta}\right),
    \end{split}
\end{gather}
and all other parameters being $\mathcal{O}(1)$.
We then take the limit by expanding all variables in powers of $\delta$ in same form as in \eqref{eqn:expand}.

\subsubsection{Leading-order model: SPM}
The leading-order current collector equations are the same as those in \eqref{eqn:high-cc:leading-order-current-collector} and therefore the potentials in the current collectors are spatially independent. It can also be shown from the first-order current collector problem that the leading-order current density is $\mathcal{I}^0=I\ts{app}$. Since the current collector potentials and the initial conditions are independent of $y-z$, each 1D electrochemical problem behaves in exactly the same way and it is sufficient to solve a single representative 1D electrochemical problem in the through-cell direction. The leading-order electrolyte and electrode components are provided in Appendix \ref{app:algebraic-expressions}, with the terminal voltage given by $V=\phi\ts{s,p}^0-\phi\ts{s,n}^0$. Additionally, the leading-order particle model is given by (\ref{eqn:leading-order-particles}). The resulting model is the commonly known SPM where a single representative particle is solved in each electrode. A step-by-step derivation of this model from the 1D DFN can be found in \cite{Marquis2019}. The thermal part of the model is given by \eqref{eqn:high-cc:leading-order-thermal} but with the heat-generation terms given by the expressions in Appendix \ref{app:high-with-diff}.

\subsubsection{Combined leading- and first-order model: SPMeCC}
The combined leading- and first-order current collector model is given by \eqref{eqn:high-cc:combined-order-current-collector} with the potentials given by the relations (\ref{eqn:high-cc:potentials}). As in Section \ref{sec:DFNCC}, we average over $y-z$, which allows us to solve for a single $y-z$-averaged 1D electrochemical model and still obtain the terminal voltage accurate to $\mathcal{O}(\delta^2)$. Additionally, since we are also considering the limit of fast diffusion in the electrolyte and high conductivity in the electrode and electrolyte, we can $x$-electrode average the particle equations as done in Section \ref{sec:2p1-SPM}. As a result, the combined leading- and first-order $y-z$ averaged electrolyte equations become
\begin{subequations}\label{eqn:SPMeCC-combined-electrolyte}
    \begin{gather}
        \mathcal{C}\ts{e} \epsilon\ts{k} \gamma\ts{e} \pdv{\YZav{c}\ts{e,k}\co}{t} = - \gamma\ts{e} \pdv{\YZav{N}\ts{e,k}\co}{x} +
        \mathcal{C}\ts{e}
        \begin{cases}
            \frac{I\ts{app}}{L\ts{n}L_yL_z}, \quad &\text{k}=\text{n}, \\
            0, \quad &\text{k}=\text{s}, \\
            -\frac{I\ts{app}}{L\ts{p}L_yL_z}, \quad &\text{k}=\text{p},
        \end{cases} \\
        \YZav{N}\ts{e,k}\co = -\epsilon\ts{k}^{\text{b}}D\ts{e}(\YZav{c}\ts{e,k}\co, \YZav{T}\co)\pdv{\YZav{c}\ts{e,k}\co}{x} +
        \mathcal{C}\ts{e}
        \begin{cases}
        \frac{x t^+ I\ts{app}}{\gamma\ts{e} L\ts{n}L_yL_z}, \quad &\text{k}=\text{n},\\
        \frac{t^+ I\ts{app}}{\gamma\ts{e}L_yL_z}, \quad &\text{k}=\text{s},\\
        \frac{(1-x) t^+ I\ts{app}}{\gamma\ts{e} L\ts{p}L_yL_z}, \quad &\text{k}=\text{p},
        \end{cases}\\
        \YZav{c}\ts{e,k}\co(x,0)=1, \quad
        \YZav{N}\ts{e,n}\co\big|_{x=0}=0, \quad
        \YZav{N}\ts{e,p}\co\big|_{x=1}=0, \\
        \YZav{c}\ts{e,n}\co\big|_{x=L\ts{n}}=\YZav{c}\ts{e,s}\co\big|_{x=L\ts{n}}, \quad
        \YZav{N}\ts{e,n}\co\big|_{x=L\ts{n}}=\YZav{N}\ts{e,s}\co\big|_{x=L\ts{n}}, \\
        \YZav{c}\ts{e,s}\co\big|_{x=1-L\ts{p}}=\YZav{c}\ts{e,p}\co\big|_{x=1-L\ts{p}}, \quad
        \YZav{N}\ts{e,s}\co\big|_{x=1-L\ts{p}}=\YZav{N}\ts{e,p}\co\big|_{x=1-L\ts{p}}.
    \end{gather}
\end{subequations}
with the combined leading- and first-order equations in a single $x$-$y$-$z$ electrode-averaged particle in each electrode given by
\begin{subequations}\label{eqn:SPMeCC:combined-order-particles}
    \begin{gather}
         \mathcal{C}\ts{k}\pdv{\XYZav{c}\ts{s,k}\co}{t} = -\frac{1}{r\ts{k}^2}\pdv{r\ts{k}}
            \left(
                r\ts{k}^2 D\ts{k}(\XYZav{c}\ts{s,k}\co, \XYZav{T}\co)
                \pdv{\XYZav{c}\ts{s,k}\co}{r\ts{k}}
            \right), \quad \kin{n, p} \\
        \pdv{\XYZav{c}\ts{s,k}\co}{r\ts{k}}\bigg|_{r\ts{k}=0}=0, \quad
        -\frac{a\ts{k}\gamma\ts{k}}{\mathcal{C}\ts{k}}
            D\ts{k}(\XYZav{c}\ts{s,k}\co, \XYZav{T}\co)
            \pdv{\XYZav{c}\ts{s,k}\co}{r\ts{k}}\bigg|_{r\ts{k}=0}=,
         \begin{cases}
         \frac{I\ts{app}}{L\ts{n}L_yL_z}, \quad & \text{k}=\text{n}, \\
         -\frac{I\ts{app}}{L\ts{p}L_yL_z}, \quad &\text{k}=\text{p},
         \end{cases} \label{eqn:lo:solidConcentration:BC} \\
         \XYZav{c}\ts{s,k}\co(r\ts{k},0) = c\ts{s,k,0}, \quad \kin{n, p}.
    \end{gather}
\end{subequations}
The combined leading- and first-order thermal problem is the same as that stated in \eqref{eqn:combined-order-temperature} but with the heat generation term replaced by the expressions in Appendix \ref{app:high-with-diff}.

It then remains to determine the terminal voltage. We employ the $y$-$z$-averaged expression for the terminal voltage \eqref{eqn:y-z-voltage} and then recognize that by using the expressions for the leading- and first-order terms in Appendix \ref{app:algebraic-expressions} and \ref{app:electrode_averaged}, we can re-write the final through-cell term as
\begin{subequations}\label{eqn:combined-order-SPMeCC-voltage}
    \begin{align}
        \left( \YZav{\phi}\ts{s,cp}\co - \YZav{\phi}\ts{s,cn}\co \right) = \XYZav{\mathcal{U}}\ts{eq}\co + \XYZav{\eta}\ts{r}\co +  \XYZav{\eta}\ts{c}\co + \XYZav{\Delta \Phi}\ts{Elec}\co + \XYZav{\Delta \Phi}\ts{Solid}\co
    \end{align}
    where
    \begin{align}
        &\XYZav{\mathcal{U}}\ts{eq}\co = U\ts{p}(\XYZav{c}\ts{s,p}\co, \XYZav{T}\co) - U\ts{n}(\XYZav{c}\ts{s,n}\co, \XYZav{T}\co), \\
        &\XYZav{\eta}\ts{r}\co = \XYZav{\eta}\ts{p}\co - \XYZav{\eta}\ts{n}\co, \\
        &\XYZav{\eta}\ts{k}\co = 2 (1 + \Theta \XYZav{T}\co) \sinh^{-1}\left(\frac{\XYZav{j}\ts{k}\co}{\XYZav{j}\ts{0,k}\co}\right)
        \quad \kin{n, p},\\
        &\XYZav{j}\ts{n}\co = \frac{I\ts{app}}{L\ts{n}},\\
        &\XYZav{j}\ts{p}\co = -\frac{I\ts{app}}{L\ts{p}}, \\
        &\XYZav{j}\ts{0,k}\co = \frac{\gamma\ts{k}}{\mathcal{C}\ts{r,k}}m\ts{k}(\XYZav{T}\co) (\XYZav{c}\ts{s,k}\co)^{1/2}  (1 - \XYZav{c}\ts{s,k}\co)^{1/2}(\XYZav{c}\ts{e,k}\co)^{1/2}, \\
        &\XYZav{\eta}\ts{c}\co = 2(1-t^+)(\XYZav{c}\ts{e,p}\co-\XYZav{c}\ts{e,n}\co),\\
        &\XYZav{\Delta\Phi}\ts{Elec}\co = - \frac{I\ts{app}}{\hat{\kappa}\kappa\ts{e}(1)}\left(\frac{L\ts{n}}{3\epsilon\ts{n}^b} + \frac{L\ts{s}}{\epsilon\ts{s}^b} + \frac{L\ts{p}}{3\epsilon\ts{p}^b} \right), \\
        &\XYZav{\Delta\Phi}\ts{Solid}\co = -\frac{I\ts{app}}{3}\left(\frac{L\ts{p}}{\sigma\ts{p}} + \frac{L\ts{n}}{\sigma\ts{n}} \right).
    \end{align}
\end{subequations}

Equations \eqref{eqn:high-cc:potentials}, \eqref{eqn:high-cc:combined-order-current-collector}, \eqref{eqn:y-z-voltage}, \eqref{eqn:SPMeCC-combined-electrolyte}, \eqref{eqn:SPMeCC:combined-order-particles}, and \eqref{eqn:combined-order-SPMeCC-voltage} form a model which we refer to as the SPMeCC (single particle model with electrolyte and current collectors). In this model, a single $x$-$y$-$z$-electrode averaged particle is solved in each electrode alongside a single $y$-$z$-averaged equation for the electrolyte dynamics. In addition, a single once-and-for-all solve of a 2D current collector model is required to account for the current collector resistance in the calculation of the terminal voltage.

\begin{comment}
\subsection{Asymptotic analysis: $\mathcal{C}\ts{e} \sim \delta$, $\alpha \sim 1$}\label{sec:alpha_delta}
\rob{I think we can do the limit $\alpha \sim \delta$ independent of the size of $\mathcal{C}\ts{e}$ i.e. we might want to discuss 2+$\bar{1}$ for any choice of DFN, SPMe etc.}
In this section we consider the limit of large conductivity in both the current collectors and solid electrode material. In particular, we consider
\begin{equation}
\sigma\ts{ck}'=\frac{\sigma_{ck}''}{\delta}, \quad \sigma\ts{k}=\frac{\sigma_{k}'}{\delta}, \quad \alpha=\delta\alpha', \quad \kin{n, p},
\end{equation}
where $\sigma\ts{k}'$, $\sigma\ts{ck}''$, and $\alpha'$ are $\mathcal{O}(1)$ quantities. We again look for a solution in terms of an asymptotic series in $\delta$, writing
\begin{equation}
\phi\ts{s,k} = \phi\ts{s,k}^0 + \delta \phi\ts{s,k}^1 + \cdots,
\end{equation}
etc.

\subsubsection{Leading-order}
Now the rescaled problem in the current collectors reads
\begin{equation}
    \nabla^2_\perp (\mathcal{V}^0 + \delta \mathcal{V}^1 + \cdots ) = -\delta \alpha' (\mathcal{I}^0 + \delta \mathcal{I}^1 + \cdots).
\end{equation}
At leading-order the potential difference must satisfy no flux boundary conditions, due to the factor of $\delta$ appearing in the right hand side of \eqref{DFNCC:voltage_tab_p}--\eqref{DFNCC:voltage_ext} upon scaling $\sigma\ts{ck}'$. Therefore the leading-order potential difference is a function of time only, $\mathcal{V}^0 = \mathcal{V}^0(t)$. The leading-order analysis holds as in Section~\ref{sec:fastdiff_asim1_LO} and, provided the initial conditions are independent of both $y$ and $z$, it follows that all of the leading-order variables are a function of at most $x$ and $t$. Moreover, from conservation of current we readily compute the leading-order current density to be $\mathcal{I}^0 = I\ts{app}/L_y$ (note that $L_z$ is, by definition, equal to one, so the leading-order through-cell currently density is the applied current divided by the current collector surface area). The governing equation for the temperature \eqref{eqn:asim1:LOtemp} is replaced with the ordinary differential equation
\begin{equation}
\frac{\rho}{\gamma\ts{th}} \dv{T^0}{t} =  \mathcal{B}\bar{Q}^0 - \frac{2 h'}{L} T^0,
\end{equation}
where the leading-order heat generation now only contains contributions due to electrochemical heating
\begin{equation}
       \bar{Q}^0 = \frac{1}{L}\bigg[ L\ts{n} j\ts{n}^0\left( \eta\ts{n}^0 + (\Theta^{-1} + T^0)\pdv{U\ts{n}}{T}\bigg\vert_{T=0} \right) + L\ts{p} j\ts{p}^0\left( \eta\ts{p}^0 + (\Theta^{-1} + T^0)\pdv{U\ts{p}}{T}\bigg\vert_{T=0} \right)\bigg].
\end{equation}
This is to be solved subject to the initial condition $T^0 = T_0$. Note that the boundary condition \eqref{DFNCC:BC:tempext} appears at $\mathcal{O}(\delta)$, that is, the heat transfer coefficient is sufficiently small so that only surface cooling on the faces of the pouch cell is significant to leading-order. There are no leading-order contributions from the Ohmic heating terms since ${\phi^0\ts{s,k}}$ is independent of space for all k. The potential difference is then given by \eqref{eqn:asim1:VLO} with the lithium concentration in the particles still governed by \eqref{eqn:lo:solidConcentration}. Since there is now no $y$ or $z$ dependence one only needs to solve \eqref{eqn:lo:solidConcentration} for a representative single particle in each electrode. Thus, in this limit the leading-order problem depends only the pseudo $r$-direction, and the model reduces to the classical Single Particle Model (SPM) with temperature effects.

\subsubsection{First-order}
At $\mathcal{O}(\delta)$, the potential difference satisfies
\begin{equation}
    \nabla_\perp^2 \mathcal{V}^1 = -\alpha'\mathcal{I}^0.
\end{equation}
It is convenient to introduce the new variable $\mathcal{W}^1 = -((\mathcal{V}^1-\tilde{\mathcal{V}}^1)/(\alpha' \mathcal{I}^0) = - ((\mathcal{V}^1-\tilde{\mathcal{V}}^1)L_y)/(\alpha' I\ts{app})$, then for a given geometry one can solve for $\mathcal{W}^1$ independently of time, and reconstruct the time dependent $\mathcal{V}^1$ for a given applied current. Here, we have again used a tilde to represent a $y$-$z$ averaged quantity. The problem for $\mathcal{W}^1$ reads
\begin{subequations}
\begin{align}
    \nabla_\perp^2 \mathcal{W}^1 &= 1 && \\
    \int_{\partial\Omega\ts{tab,p}}\nabla_\perp\mathcal{W}^1\cdot\boldsymbol{n} \dd{x}&=  \frac{L_y}{\alpha'\sigma\ts{cp}''} \quad &&(y,z)\in\partial\hat{\Omega}\ts{tab,p}\big/\partial\hat{\Omega}\ts{tab,n}, \\
    \int_{\partial\Omega\ts{tab,n}}\nabla_\perp\mathcal{W}^1\cdot\boldsymbol{n} \dd{x}&=  \frac{L_y}{\alpha'\sigma\ts{cn}''} \quad &&(y,z)\in\partial\hat{\Omega}\ts{tab,n}\big/\partial\hat{\Omega}\ts{tab,p}, \\
    \nabla_\perp\mathcal{W}^1\cdot\boldsymbol{n} &= 0 \quad &&(y,z)\in\partial\hat{\Omega}\ts{ext,p}\cap\partial\hat{\Omega}\ts{ext,n}, \\
    \tilde{\mathcal{W}}^1 &= 0.  &&
\end{align}
\end{subequations}
We then recover the correction to the potential difference through the relation
\begin{equation}\label{eqn:next_order_voltage}
    \mathcal{V}^1 = \tilde{\mathcal{V}}^1 - \alpha' \mathcal{I}^0 \mathcal{W}^1
\end{equation}
Therefore, to obtain $\mathcal{V}^1$ in this limit, one only needs to determine the $y$-$z$ average of the correction to the potential difference $\tilde{\mathcal{V}}^1$.  We first note that, by conservation of current, the $y$-$z$ average of the $\mathcal{O}(\delta)$ component of the current is zero, i.e. $\tilde{\mathcal{I}}^1 = 0$, and that the $y$-$z$ average of the $x$-averaged electrolyte variables remains unchanged
\begin{equation}
 \tilde{\bar{\phi}}\ts{e,k}^1 = \bar{\phi}\ts{e,k}^1,  \quad \tilde{\bar{c}}\ts{e,k}^1 = \bar{c}\ts{e,k}^1,
\end{equation}
where a tilde and an overbar are used to indicate that the quantity is averaged over $y$ and $z$, and the $x$ direction of $\Omega\ts{k}$. We then average \eqref{eqn:od:electrode_av_con} over $y$ and $z$, which results in no-flux boundary conditions in the problem for $\tilde{\bar{c}}\ts{k}^1$. It is then clear that the volume-averaged correction to the particle concentration is zero, i.e. $\tilde{\bar{c}}\ts{k}^1 = 0$. Then, from \eqref{eqn:asim1:V1} we find the average correction to the potential difference to be
\begin{equation}\label{eqn:asimdelta:avgV1}
    \begin{split}
        \tilde{\mathcal{V}^1} &= \bar{\phi}\ts{e,p}^1 - \bar{\phi}\ts{e,n}^1 \\
    &\quad - \frac{2\tilde{\bar{j}}\ts{0,p}^1}{j\ts{0,p}^0 L\ts{p}}\tanh{\left(\frac{\eta\ts{p}^0}{2(1 + \Theta T^0)}\right)} + \frac{2 \tilde{\bar{j}}\ts{0,n}^1}{j\ts{0,n}^0 L\ts{n}}\tanh{\left(\frac{\eta\ts{n}^0}{2(1 + \Theta T^0)}\right)} \\
    &\quad + \pdv{U\ts{p}}{T} (c\ts{s,p}^0,T^0)\tilde{T}^1 - \pdv{U\ts{n}}{T} (c\ts{s,n}^0,T^0)\tilde{T}^1 \\
    &\quad - \frac{\mathcal{I}^0}{3}\left( \frac{L\ts{p}}{\sigma\ts{p}'} + \frac{L\ts{n}}{\sigma\ts{n}'}\right),
    \end{split}
\end{equation}
where
\begin{equation}
    \tilde{\bar{j}}\ts{0,k}^1 = \left[ \frac{j\ts{0,k}^0}{2} \bar{c}\ts{e,k}^1 + \frac{j\ts{0,k}^0}{m\ts{k}(T^0)}m\ts{k}'(T^0)\tilde{T}^1\right]_{r\ts{k}=1}.
\end{equation}
\rob{Scott, could you add in an explanation of the steps of going from this to the expression you have for the voltage losses due to various physical effects?}

The governing equation for the volume-averaged temperature is found by integrating \eqref{eqn:asim1:temp1} in $y$ and $z$ over the whole domain, the result being
\begin{equation}
    \mathcal{C}\ts{th} \rho \pdv{T^1}{t} =  \mathcal{B}\bar{Q}^1 - \frac{2h'}{L}T^1 - 2(1+L_y)h'T^0,
\end{equation}
with the initial condition $\tilde{T}^1 \big\vert_{t=0} = 0$.

In order to obtain the potential difference as a function of space we then substitute the result \eqref{eqn:asimdelta:avgV1} into \eqref{eqn:next_order_voltage} along with the solution $\mathcal{W}^1$. To recover the distribution of current density, one also needs to solve the full problem for the temperature distribution $T^1$, and for the $x$-averaged correction to particle concentration $\bar{c}\ts{s,k}^1$. Then the correction to the current density $\mathcal{I}^1$ and potential difference $\mathcal{V}^1$ are related by \eqref{eqn:asim1:V1}, with $\mathcal{I}^0$ now a known function of time.

\subsection{Reduced order model: SPMeCC}
Using our results from Section~\ref{sec:alpha_delta} we may obtain an expression for the terminal voltage which is correct to $\mathcal{O}(\delta)$ for which it is only necessary to solve two time-independent Poisson problems for $\mathcal{W}^1$ and $\psi$, two ODEs for the leading- and first-order volume-averaged temperature, and two PDEs for the lithium concentration in a representative particle in each electrode. Thus, we have derived an extended Single Particle Model which accounts for the geometry dependent Ohmic losses in the current collectors, as well as Ohmic losses in the electrolyte, and temperature effects. The model derived in the previous section holds when the electrolyte can be considered to be in steady state. However, it is a simple extension to rescale time as $t=\delta \hat{t}$ so that we capture initial transient effects in the electrolyte. This extension results in an additional PDE which determines the time evolution of $c\ts{e,k}^1$.

The terminal voltage $V = V^0 + \delta V^1$ is given by
\begin{align}
    V^0 &= \mathcal{V}^0(t), \\
    \nonumber
    V^1 &= \left.\phi\ts{s,cp}^1\right|\ts{tab,p} - \left.\phi\ts{s,cn}^1\right|\ts{tab,n} = \tilde{\phi}\ts{s,cp} - \tilde{\phi}\ts{s,cn} +  (\left.\phi\ts{s,cp}^1\right|\ts{tab,p} - \tilde{\phi}\ts{s,cp}) - (\left.\phi\ts{s,cn}^1\right|\ts{tab,n} - \tilde{\phi}\ts{s,cn}) \\
    & = \tilde{\mathcal{V}}^1(t) + (\left.\phi\ts{s,cp}^1\right|\ts{tab,p} - \tilde{\phi}\ts{s,cp}) - (\left.\phi\ts{s,cn}^1\right|\ts{tab,n} - \tilde{\phi}\ts{s,cn}).
\end{align}
Calculating the quantities in the final two terms in brackets gives a result which may be written as a linear resistor
\begin{equation}
    (\left.\phi\ts{s,cp}^1\right|\ts{tab,p} - \tilde{\phi}\ts{s,cp}) - (\left.\phi\ts{s,cn}^1\right|\ts{tab,n} - \tilde{\phi}\ts{s,cn}) = - I\ts{app}R\ts{CC},
\end{equation}
where
\begin{equation}
 R\ts{CC} =   \frac{1}{\sigma\ts{cn}''L\ts{cn}+ \sigma\ts{cp}''L\ts{cp}}\left( \frac{\alpha'}{L_y}\left( \sigma\ts{cn}''L\ts{cn}\mathcal{W}^1|\ts{tab,p} + \sigma\ts{cp}''L\ts{cp}\mathcal{W}^1|\ts{tab,n} \right) -  (\psi|\ts{tab,p}-\psi|\ts{tab,n}) \right).
\end{equation}
We then define the average Ohmic losses in the current collector to be $\Delta \Phi_{\text{CC}} = -\delta I\ts{app}R\ts{CC}$ so that the terminal voltage is given by
\begin{equation}
    V = (\mathcal{V}^0 + \delta \tilde{\mathcal{V}}^1) + \Delta\Phi_{\text{CC}}.
\end{equation}

\newpage

We now summarise the reduced model which we refer to as the Single Particle Model with electrolyte and Current Collectors (SPMeCC) with temperature effects.

\rob{I'm not a huge fan of the appearance of this bold/italic layout for summarising the equations, but happy to be convinced to keep it}


\begin{subequations}\label{SPMeCC_effectiveresistance}
    \begin{align}
    \intertext{\textbf{Time Independent Geometric Problems}}
    \intertext{$\psi$ \emph{problem}:}
    \nabla_\perp^2 \psi &= 0, && \\
    \int_{\partial\Omega\ts{tab,p}}\nabla_\perp\psi\cdot\boldsymbol{n}\dd{x}  &= -L\ts{cp}, &&  \\
     \int_{\partial\Omega\ts{tab,n}}\nabla_\perp\psi\cdot\boldsymbol{n} \dd{x} &= L\ts{cn}, && \\
    \nabla_\perp\psi\cdot\boldsymbol{n} &= 0 \quad &&(y,z)\in\partial\Omega_{\text{ext},p}\cap\partial\Omega_{\text{ext},n}.
    \intertext{$\mathcal{W}^1$ \emph{problem}:}
    \nabla_\perp^2 \mathcal{W}^1 &= 1, && \\
    \int_{\partial\Omega\ts{tab,p}}\nabla_\perp\mathcal{W}^1\cdot\boldsymbol{n} \dd{x}&=  \frac{L_y}{\alpha'\sigma\ts{cp}''} &&, \\
    \int_{\partial\Omega\ts{tab,n}}\nabla_\perp\mathcal{W}^1\cdot\boldsymbol{n} \dd{x}&=  \frac{L_y}{\alpha'\sigma\ts{cn}''} , \\
    \nabla_\perp\mathcal{W}^1\cdot\boldsymbol{n} &= 0 \quad &&(y,z)\in\partial\hat{\Omega}\ts{ext,p}\cap\partial\hat{\Omega}\ts{ext,n}, \\
    \tilde{\mathcal{W}}^1 &= 0.  &&
    \end{align}
\end{subequations}
\begin{subequations}\label{SPMeCC_ODEs}
    \begin{align}
    \intertext{\textbf{0D Time Dependent Problems}}
    \intertext{\emph{Leading-order $x$-independent temperature}:}
    \mathcal{C}\ts{th} \rho \dv{T^0}{t} &=  \mathcal{B}\bar{Q}^0 - \frac{2 h'}{L} T^0, &&\\
    T^0 \big\vert_{t=0} &= T_0, && \\
    \intertext{\emph{First-order volume-averaged temperature}:}
    \nonumber
     \mathcal{C}\ts{th} \rho \dv{\tilde{T}^1}{t} &=  \mathcal{B}\tilde{\bar{Q}}^1 - \frac{2 h'}{L} \tilde{T}^1 - 2(1+L_y)h'T^0 && \\
     \tilde{T}^1 \big\vert_{t=0} &= 0. &&
    \end{align}
\end{subequations}
\begin{subequations}\label{SPMeCC_PDEs}
    \begin{align}
    \intertext{\textbf{1D Time Dependent Problems}}
    \intertext{\emph{Leading-order particle concentration}:}
     \mathcal{C}\ts{k}\pdv{c\ts{s,k}^0}{t} &= -\frac{1}{r\ts{k}^2}\pdv{r\ts{k}}\left(r\ts{k}^2 N\ts{s,k}^0\right), \quad N\ts{s,k}^0 = D\ts{k}(c\ts{s,k}^0, T^0) \pdv{c\ts{s,k}^0}{r\ts{k}}, && \kin{n, p} \\
     N\ts{s,k}^0\bigg|_{r\ts{k}=0} &= 0, \quad  \kin{n p}, \ \ \frac{a\ts{k}\gamma\ts{k}}{\mathcal{C}\ts{k}}N\ts{s,k}^0\bigg|_{r\ts{k}=1} =
     \begin{cases}
     \frac{\mathcal{I}^0}{L\ts{n}}, \quad & \text{k}=\text{n}, \\
     -\frac{\mathcal{I}^0}{L\ts{p}}, \quad &\text{k}=\text{p},
     \end{cases}
     &&\\
     c\ts{s,k}^0(r\ts{k},0) &= c\ts{s,k,0}, && \kin{n, p}.
    \intertext{$\mathcal{O}(\delta)$ \emph{electrolyte concentration}:}
    \delta \mathcal{C}\ts{e} \gamma\ts{e}\epsilon\ts{k}\pdv{c\ts{e,k}^1}{t} &= -\gamma\ts{e}\pdv{N\ts{e,k}^1}{x} +
    \begin{cases}
    \mathcal{C}\ts{e}'\frac{\mathcal{I}^0}{L\ts{n}}, \quad &\text{k}=\text{n} \\
    0, \quad &\text{k}=\text{s} \\
    -\mathcal{C}\ts{e}' \frac{\mathcal{I}^0}{L\ts{p}}, \quad &\text{k}=\text{p}
    \end{cases}
    && \kin{n, s, p}, \\
    \label{eqn:SPMe:electrolyte:flux}
    N\ts{e,k}^1 &= -\epsilon\ts{k}^{\text{b}} D\ts{e}(1, T^0) \pdv{c^1\ts{e,k}}{x} +     \begin{cases}
     x\frac{\mathcal{C}\ts{e}' t^+}{\gamma\ts{e}}\frac{\mathcal{I}^0}{L\ts{n}}, \quad &\text{k}=\text{n} \\
     \frac{\mathcal{C}\ts{e}' t^+}{\gamma\ts{e}}\mathcal{I}^0, \quad &\text{k}=\text{s} \\
     (1-x)\frac{\mathcal{C}\ts{e}' t^+}{\gamma\ts{e}} \frac{\mathcal{I}^0}{L\ts{p}}, \quad &\text{k}=\text{p}
    \end{cases}, && \kin{n, s, p}, \\
    N\ts{e,n}^1\big|_{x=0} &= 0, \quad N\ts{e,p}^1\big|_{x=1}=0,  &&\\
    c\ts{e,n}^1|_{x=L\ts{n}}&=c\ts{e,s}^1|_{x=L\ts{n}}, \quad N\ts{e,n}^1\big|_{x=L\ts{n}}=N\ts{e,s}^1\big|_{x=L\ts{n}}, && \\
    c\ts{e,s}^1|_{x=1-L\ts{p}}&=c\ts{e,p}^1|_{x=1-L\ts{p}}, \quad N\ts{e,s}^1\big|_{x=1-L\ts{p}}=N\ts{e,p}^1\big|_{x=1-L\ts{p}}. &&
    \end{align}
\end{subequations}
\begin{subequations}\label{SPMeCC_voltage}
    \begin{align}
    \intertext{\textbf{Voltage}}
    \intertext{\emph{Terminal voltage}:}
        &V = \mathcal{U}\ts{eq} + \eta\ts{r} + \eta\ts{c} + \Delta\Phi\ts{elec} + \Delta\Phi\ts{solid} + \Delta\Phi\ts{CC}.
    \intertext{\emph{Potential difference}:}
    &\mathcal{V} = \tilde{\mathcal{V}}- \alpha \mathcal{I}^0 \mathcal{W}^1, \\
    & \tilde{\mathcal{V}} = \mathcal{U}\ts{eq} + \eta\ts{r} + \eta\ts{c} + \Delta\Phi\ts{elec} + \Delta\Phi\ts{solid}.
     \intertext{\emph{Terminal voltage components}:}
     & \mathcal{U}\ts{eq} = U\ts{p}(c\ts{s,p}^0, T^0)\big|_{r\ts{p}=1} - U\ts{s,n}(c\ts{n}^0, T^0)\big|_{r\ts{n}=1} + \delta \left( \pdv{U\ts{p}}{T} (c\ts{s,p}^0,T^0)\tilde{T}^1 - \pdv{U\ts{n}}{T} (c\ts{s,n}^0,T^0)\tilde{T}^1 \right), \\
     &\eta\ts{r} = -(1 + \Theta T^0)\sinh^{-1}\left(\frac{I_{\text{app}}}{\tilde{\bar{j}}\ts{0,p} L\ts{p} L_y}\right)
     -2(1 + \Theta T^0)\sinh^{-1}\left(\frac{I_{\text{app}}}{\tilde{\bar{j}}\ts{0,n} L\ts{n} L_y}\right), \\
     \label{eqn:SPMe:negative_exchange}
     &\tilde{\bar{j}}\ts{0,n} =  \frac{1}{L\ts{n}}\int_0^{L\ts{n}} \frac{\gamma\ts{n}}{\mathcal{C}\ts{r,n}} m\ts{n}(T^0 + \delta T^1) (c\ts{s,n}^0)^{1/2}(1-c\ts{s,n}^0)^{1/2} (1+\delta c\ts{e,n}^1 )^{1/2} \dd{x}, \\
     \label{eqn:SPMe:positive_exchange}
    &\tilde{\bar{j}}\ts{0,p} =  \frac{1}{L\ts{p}}\int_{1-L\ts{p}}^{1} \frac{\gamma\ts{p}}{\mathcal{C}\ts{r,p}} m\ts{p}(T^0 + \delta T^1) (c\ts{s,p}^0)^{1/2}(1-c\ts{s,p}^0)^{1/2} (1+\delta c\ts{e,p}^1 )^{1/2} \dd{x}, \\
     \label{eqn:SPMe:concentration:overpotential}
     &\eta\ts{c} =  2 \delta (1-t^+)(1 + \Theta T^0)\left(\bar{c}\ts{e,p}^1 - \bar{c}\ts{e,n}^1\right), \\
     &\Delta \Phi\ts{elec}= -\frac{\delta \mathcal{C}\ts{e}' I_\text{app}}{\gamma\ts{e} \kappa\ts{e}(1, T^0)L_y}\left(\frac{L\ts{n}}{3\epsilon\ts{n}^{\text{b}}} + \frac{L_s}{\epsilon_{s}^{\text{b}}} + \frac{L\ts{p}}{3\epsilon\ts{p}^{\text{b}}} \right),
     \label{eqn:SPMe:electrolyte_ohmic_losses} \\
     &\Delta \Phi\ts{solid} =  -\frac{I_{\text{app}}}{3 L_y}\left(\frac{L\ts{p}}{\sigma\ts{p}} + \frac{L\ts{n}}{\sigma\ts{n}} \right), \\
     & \Delta \Phi_{\text{CC}} = - \delta I\ts{app}R\ts{CC}.
     \end{align}
\end{subequations}

\end{comment}
\end{comment}
